Feature-Interaction Aware Configuration Prioritization for Configurable Code

Unexpected interactions among features induce most bugs in a configurable software system. Exhaustively analyzing all the exponential number of possible configurations is prohibitively costly. Thus, various sampling techniques have been proposed to systematically narrow down the exponential number of legal configurations to be analyzed. Since analyzing all selected configurations can require a huge amount of effort, fault-based configuration prioritization, that helps detect faults earlier, can yield practical benefits in quality assurance. In this paper, we propose CoPro, a novel formulation of feature-interaction bugs via common program entities enabled/disabled by the features. Leveraging from that, we develop an efficient feature-interaction aware configuration prioritization technique for a configurable system by ranking the configurations according to their total number of potential bugs. We conducted several experiments to evaluate CoPro on the ability to detect configuration-related bugs in a public benchmark. We found that CoPro outperforms the state-of-the-art configuration prioritization techniques when we add them on advanced sampling algorithms. In 78% of the cases, CoPro ranks the buggy configurations at the top 3 positions in the resulting list. Interestingly, CoPro is able to detect 17 not-yet-discovered feature-interaction bugs.

==> abstract.tex <==
\begin{abstract}
%In a configurable software system, unexpected interactions among
%features might induce bugs. The exhaustive analysis approach is
%prohibitively costly because of the exponential number of all possible
%configurations. The sampling techniques to select a subset of
%configurations for testing are still limited because they do not
%examine the source code and do not provide an assessment of potential
%buggy configurations. In this paper, we propose {\tool}, a novel
%formulation of feature-interaction bugs via common program entities
%enabled/disabled by the features. Leveraging from that, we develop
%efficient feature-interaction-aware configuration prioritization
%technique for a configurable system by ranking the configurations
%according to their total number of potential bugs. We conducted
%several experiments to evaluate {\tool} in two complementary settings:
%detecting configuration-related bugs in a benchmark and real-world
%open-source systems. We found that {\tool} outperforms the other
%techniques. In 85\% of the cases, it ranks the buggy
%configurations at the top 3 positions. Interestingly, it is able to
%detect 17 not-yet-discovered, high-degree,
%feature-interaction~bugs.
%
%Old version
%
%Unexpected interactions among features induce most bugs in a
%configurable software system. Exhaustively analyzing all exponential
%number of possible configurations is~prohibitively costly.  Thus,
%various sampling techniques have been proposed to systematically
%narrow down the exponential number of configurations to be tested.
%%
%Since testing all selected configurations can require a huge amount of
%effort, fault-based configuration prioritization, that helps detect
%faults earlier, can yield practical benefits in quality assurance. In
%this paper, we propose {\tool}, a novel formulation of
%feature-interaction bugs via common program entities enabled/disabled
%by the features. Leveraging from that, we develop an efficient
%feature-interaction-aware configuration prioritization technique for a
%configurable system by ranking the configurations according to their
%total number of potential bugs. We conducted several experiments to
%evaluate {\tool} on the ability to detect configuration- related bugs
%in a public benchmark. We found that {\tool} outperforms the
%state-of-the-art configuration prioritization techniques.
%%when we add them on popular sampling algorithms.
%Interestingly, it is able to detect 17 not-yet-discovered
%feature-interaction bugs.

Unexpected interactions among features induce most bugs in a
configurable software system. Exhaustively analyzing all exponential
number of possible configurations is~prohibitively costly. Thus,
various sampling methods have been proposed to systematically
narrow down the exponential number of configurations to be tested.
%
Since testing all selected configurations can require a huge amount of
effort, fault-based configuration prioritization, that helps detect
bugs earlier, can yield practical benefits in quality assurance. In
this paper, we propose {\tool}, a novel formulation of
feature-interaction bugs via common program entities enabled/disabled
by the features. Leveraging from that, we develop an efficient
feature-interaction-aware configuration prioritization technique for
configurable systems by ranking configurations according to their total number of potential bugs. We conducted several experiments to evaluate {\tool}
%on the ability to detect configuration-related bugs
%in bug detection
on a public benchmark. We found that {\tool} outperforms the
state-of-the-art configuration prioritization methods. Interestingly,
it is able to detect 17 not-yet-discovered feature-interaction bugs.
\end{abstract}


==> approach.tex <==
\section{Approach}

%To improve the efficiency of configuration testing,
We propose {\tool}, a novel approach for configuration prioritization 
based on detecting feature-interaction bugs. \textit{Unlike the SP 
which does not examine the nature of potential bug-inducing feature 
interactions}, \textbf{we analyze the code to detect feature 
interactions via operations on the program entities that are shared 
between features}. Those operations, when the features are enabled 
or disabled, potentially create a violation(s) of the program semantics,
which helps identify interaction bugs. 
%
%An example of a violation is that a feature disables the declaration of an entity while enabling one of its references. 
%
The suspicious score of a variant is determined via the total number of
potential bugs. The variants are ranked according to their suspicious scores.
%Tien
%, which helps testing and debugging activities more efficient.
%
%

\textbf{Feature}. In {\tool}, a feature in configurable code is
considered to be implemented via the operations including
\textit{declare, assign, use}, and \textit{destruct} on a set of
program entities including variables and functions. For example,
feature \texttt{L} is implemented via operation \textit{declare} on
the function \texttt{of\_platform\_populate} and variable
\texttt{node}.

%Link the notion of feature and option
\textbf{Feature Interaction}. Features interact with one another
through their operations on the shared program entities depending on
the manners that the shared entities operate in the features. In Fig.
\ref{example1}, \texttt{of\_platform\_p\-opulate} is {\em declared} in  
\texttt{L}, and \texttt{L} interacts with \texttt{Z} where
the function is {\em used}. In a configurable code, enabling or
disabling a feature is determined by certain configuration options' 
selection. In Fig. \ref{example1}, \texttt{L} is enabled if 
\texttt{CONFIG\_SPARC=F}, and \texttt{Z} is enabled when 
\texttt{CONFIG\_TWL4\-030\_CORE} and \texttt{CONFIG\_OF\_DEVICE} 
are \texttt{true}. In fact, an option is used to configure source code 
of configurable system, such that the option's value determines the 
presence/absence of segments of code. Thus, we detect feature interactions 
via common entities operating in thecode segments determined by option 
selections. For example, because \texttt{of\_platform\_populate} is 
respectively \textit{declared} and \textit{used} in the code segments 
determined by \texttt{CONFIG\_SPARC=F} and \texttt{CONFIG\_OF\_DEVICE=T}, 
there is a potential \textit{declare-use} interaction among features.  
In general, with the set of 4 operations, we define 9 kinds of feature
interaction such as \textit{declare-declare}, \textit{declare-use} and
\textit{assign-use} (7 of total 16 combinations are redundant, e.g.,
\textit{declare-use} and \textit{use-declare}) that are statically
detected through program entities shared between features.

%
%

\textbf{Configuration Prioritization}. To prioritize a set of 
configurations, our algorithm assigns a suspicious score 
to all configurations. The score of a configuration is determined via 
the number of \textit{suspicious selections} that potentially cause 
interaction bugs and flaws in different kinds such as \textit{use without 
assignment} and \textit{memory leak} that the variant 
might have. In {\tool}, suspicious option selections are identified 
based on the related kind of feature interaction. For example, 
\texttt{\{CONFIG\_SPARC=T, CONFIG\_OF\_DEVICE=T\}} are considered 
as suspicious because the related \textit{declare-use} interaction, 
and they potentially cause a \textit{use without declaration} bug.

%Running example
For example, by running {\tool}, there are 4 suspicious selections: 
\begin{compactitem}
\item \texttt{\{CONFIG\_SPARC=T, CONFIG\_OF\_DEVICE=T\}}
\item \texttt{\{CONFIG\_OF\_IRQ=F, CONFIG\_TWL4030\_CORE=T\}}
\item \texttt{\{CONFIG\_SPARC=T, CONFIG\_TWL4030\_CORE=T\}}
\item \texttt{\{CONFIG\_IRQ\_DOMAIN=F, CONFIG\_OF\_IRQ=F\}}
\end{compactitem}
%
and a much better test schedule, where {\tool}'s top-ranked configuration 
discovers both above feature interaction bugs.
%In this example, if the feature using the variable is enabled, 
%while the feature declaring the variable is disabled, the program 
%would not compile (due to \textit{using an undeclared variable}). 
%Thus, it is clear that the variant in which the first feature is 
%disabled and the second is enabled, is more suspicious than both 
%of them enabled or disabled. In general, the more bugs the 
%variant might have, the more suspicious the variant is. Finally, 
%the variants are ranked according to the suspiciousness of 
%variants.

==> comparison_apfd_src.tex <==
\begin{table}[h]
\small
\caption{Comparison Results}
\label{apfd_table}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{CoPo} & \multicolumn{2}{c|}{SP} & \multicolumn{2}{c|}{Random} \\ \cline{2-7} 
 & APFD & AVGR & APFD & AVGR & APFD & AVGR \\ \hline
Pairwise & 0.93 & 1.58 & 0.75 & 4.03 & 0.68 & 5.23 \\ \hline
Three-wise & 0.95 & 2.45 & 0.89 & 4.74 & 0.82 & 8.00 \\ \hline
OneEnabled & 0.92 & 10.93 & 0.70 & 27.67 & 0.63 & 36.37 \\ \hline
OneDisabled & 0.86 & 14.76 & 0.57 & 38.21 & 0.60 & 37.34 \\ \hline
\end{tabular}
\end{table}


==> comparison_table.tex <==
\begin{table}[]
\centering
\caption{{\tool}' Performance versus $Random$ and $SP$}
\label{comparision_table}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{} 	 & \multicolumn{2}{l|}{{\tool} vs. $Random$} 		& \multicolumn{2}{l|}{{\tool} vs. $SP$} \\ \cline{2-5} 
                     & \multicolumn{1}{c|}{W/D/L} & \begin{tabular}[c]{@{}l@{}}Avg W/L\\ margin rank\end{tabular} & W/D/L & \begin{tabular}[c]{@{}l@{}}Avg W/L\\ margin rank\end{tabular} \\ \hline
Pair-wise			&	36/9/1		&	4.19/1.00	&	34/5/7		& 3.03/1.71		\\ \hline
Three-wise			& 	34/9/3		&   6.88/6.67   	&   33/6/7      	& 3.70/4.71    	\\ \hline
Four-wise        	&   32/5/9     	&   9.13/9.5   	&   25/16/5     	& 5.52/8.80		\\ \hline
Five-wise        	&   31/6/9     	&   9.29/8.00   	&   28/13/5     	& 5.26/6.00		\\ \hline
%Sixwise         	&               	&              	&               	&       			\\ \hline
One-Enabled      	&   17/52/1		&   46.11/16.00 	&   16/16/2		& 36.81/15.50	\\ \hline
One-Disabled     	&   20/15/6   	&   44.45/5.17	&   18/16/7		& 58.89/24.14 	\\ \hline
\begin{tabular}[c]{@{}l@{}}MostEnabled\\ Disabled\end{tabular} & 10/34/2 & 1.00/1.00                                            &   4/38/4             & 1.00/1.00        \\ \hline
\begin{tabular}[c]{@{}l@{}}Statement\\ -coverage\end{tabular}  & 20/20/6 & 44.45/5.17 & 18/21/7   &                                                              58.89/24.14 \\ \hline
\end{tabular}
\end{table}

%\begin{table}[]
%\tabcolsep 5pt
%\centering
%\caption{{\tool}' running time}
%\label{running_time}
%\begin{tabular}{|l|l|l|l|l|l|l|l|}
%\hline
%                                                             & Pairwise & Threewise & Fourwise & Fivewise & OneEnabled & OneDisabled & \begin{tabular}[c]{@{}l@{}}Statement\\ -coverage\end{tabular} \\ \hline
%\begin{tabular}[c]{@{}l@{}}Running \\ time (ms)\end{tabular} &          &           &          &          &            &             &                                                               \\ \hline
%\end{tabular}
%\end{table}

==> discussion.tex <==
\subsection{Discussion}


==> discussion_src.tex <==
%Discuss about the scalability of the approach

\textbf{Conclusion}. 
%%----> Move to abstract
We introduce {\tool}, an efficient feature-interaction-aware
configuration prioritization technique for configurable systems. The
novel idea of {\tool} is the code analysis to detect interactions
between features and use them to rank configurations.
%
Currently, we formulate feature interaction statically through a
complete set of operations on the entities shared between
features. More sophisticated interactions relevant to pointers and
external data such as files or databases can be detected by using
other data structures in the same principle and other analyses.

%In summary, our main contributions
%include: 1) a novel formulation of feature-interaction; 2) an efficient
%feature-interaction-aware configuration prioritization technique for
%configurable systems; and 3) an empirical evaluation showing {\tool}'s
%effectiveness over the existing approaches.


==> disscussion.tex <==
%Discuss about the scalability of the approach

Currently, we formulate feature interaction statically through the completed set of operations on the entities that are shared between features. The  interactions relevant to pointers and external data such as files or databases can be detected by using different data structures in the same principle and use dynamic analysis.

==> intro_src.tex <==
\section{Problem Statement \& Background}
\label{sec:intro}
%cut
%Almost all software systems enable developers to configure systems to
%different environments and requirements. 
A configurable system can provide a very large number of \textit{configuration options} that 
are used to control different \textit{features} to tailor systems' properties to the needs of users and the requirements of 
customers. 
%For example, the Linux Kernel supports more than 26,000 compile-time 
%configuration options, that can be configured to generate specific kernel 
%\textit{variants} for billions of scenarios.
%
Features can interact with others in some non-trivial manners to 
modify or influence the functionality of one
another~\cite{Zave:2003:EFE:766951.766969}.  Unexpected interactions
might induce bugs. In facts, most configuration-related faults are
caused by feature interactions 
\cite{Abal:2018:VBH:3177743.3149119,
  Garvin:2011:FIF:2120102.2120918,Medeiros:2016:CSA:2884781.2884793}.
Bugs in a particular variant can be detected by traditional
methods. Unfortunately, such tools cannot be directly applied to
configurable systems. Furthermore, exhaustively analyzing a system is
infeasible due to the exponential number of configurations.
%
%In practice, configuration testing is usually performed in a manual
%and ad-hoc manner by unsystematically selecting common variants for analysis. 
%Even worse, configuration-related bugs are~discovered by users who has
%suffered the consequences of those defects.

%To systematically perform quality assurance for a configurable
%system,
%To systematically test a configurable system,
Researchers have proposed several techniques to narrow the
configuration space {\em by eliminating invalid configurations that
  violate the feature model} of the system, which defines the feasible
configurations via the constraints among the features~\cite{kastner2012virtual,kang1990feature,Gruler:2008:MMC:1424547.1424557, Post:2008:CLV:1642931.1642971,Classen:2010:MCL:1806799.1806850,Classen:2011:SMC:1985793.1985838}. However, the
number of configurations is still exponential. To address this problem, researchers introduce
various {\em configuration selection} strategies. The popular
strategies include the sampling algorithms~\cite{Medeiros:2016:CSA:2884781.2884793, Perrouin:2010:AST:1828417.1828490,Oster:2010:AIP:1885639.1885658,johansen-splc12,Tartler:2012:CCA:2094091.2094095,Marijan:2013:PPT:2491627.2491646, Abal:2014:VBL:2642937.2642990} such as \textit{combinatorial
  interaction testing}~\cite{Perrouin:2010:AST:1828417.1828490,Oster:2010:AIP:1885639.1885658,johansen-splc12,Marijan:2013:PPT:2491627.2491646}, \textit{one-enabled}~\cite{Medeiros:2016:CSA:2884781.2884793}, \textit{one-disabled}~\cite{Abal:2014:VBL:2642937.2642990},
to reduce the number of variants to be tested.
%
Still, \textit{those algorithms assume the chances of detecting
  interaction bugs are the same for all those combinations}. Thus,
interaction faults might be discovered only after the last variants in
such samples is tested. Finally, to detect defects in the system in an
effective manner, after configuration selection, the selected {\em set
  of configurations need to be prioritized} for
testing~\cite{Al-Hajjaji:2014:SPS:2648511.2648532}.

%In this approach, the selected following variant has the minimum similarity
%with the previous variants.
%


==> kway.tex <==
\begin{table}[h]
\small
\centering
\tabcolsep 3pt
\caption{The configurations sampled by 4-wise algorithm}
\label{kway}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\#          & OF\_IRQ        & IRQ\_DOMAIN   & OF\_DEVICE     & TWL4030\_CORE          & SPARC \\ \hline
1           & T  	      & T 		  & T  			& T  			& F                                            \\ \hline
2          	& F           & F          & F           	& F          	& T                                                    \\ \hline
%3          & F           & T          & F          	& F           	& T                                                    \\ \hline
4           & \textbf{F}  & \textbf{T} & \textbf{T} & \textbf{T}   & \textbf{F}                                                     \\ \hline
%5          & T           & T         & F           	& T           	& T                                                    \\ \hline
6           & \textbf{T}           & \textbf{T}         & \textbf{T}  & \textbf{T}       & \textbf{T}                                                    \\ \hline
7           & \textbf{F}	 & \textbf{T}& \textbf{T}	& \textbf{T}    & \textbf{T}                                                    \\ \hline
%8           & F & T & F   & T   & T                                                    \\ \hline
%9           & T          & T          & T           	& F          	& F                                                    \\ \hline
%10          & F 			& T 			& F  			& F 				& F                                            \\ \hline
%11 			& T 			& T 			& F 				& T  			& F                                            \\ \hline
%12          & F			&T			&T				&T				&F                                                    \\ \hline
%13          & T&F&T&F&F                                                    \\ \hline
%14          & F&F&T&F&F                                                    \\ \hline
%15          & F&F&F&F&F                                                    \\ \hline
%16          & T&F&F&F&F                                                    \\ \hline
%17 			& T&F&F&T&F  \\ \hline
%18          & T&F&T&T&F                                                     \\ \hline
%19          & F&F&F&T&F \\ \hline
%20 			& F&F&T&T&F \\ \hline
\end{tabular}
\end{table}


==> motivation.tex <==
%\vspace{-0.145in}
\section{Motivation and Observation}
The state-of-the-art method on configuration prioritization, similarity-based prioritization 
(SP)~\cite{Al-Hajjaji:2014:SPS:2648511.2648532} is still limited in detecting 
feature interaction bugs. This approach aims to cover as many
different features, but does not examine the nature of interaction between them, 
which is the key aspect causing interaction bugs in a variant.

To illustrate the problem, let us consider a simplified version of
two feature-interaction bugs in the Linux kernel in Figure 
\ref{example1}:

\begin{compactitem}[\textbullet]
\item A compile-time error occurs (\textit{using an undeclared function} on
  line~24) in the configurations in which \texttt{CONFIG\_TWL4030\-\_CORE,
    CONFIG\_OF\_DEVICE, and CONFIG\_SPARC} are enabled.

\item A run-time error occurs (\textit{dereferencing a \texttt{NULL} variable}, line~12)
~in the configurations where \texttt{CONFIG\_TWL4030\-\_CORE,
    CONFIG\_OF\_D\-EVICE} are enabled, \texttt{CONFIG\_SPARC},
  \texttt{CONFIG\_OF\_IRQ} are disabled.
\end{compactitem}

SP is based on the idea 
that dissimilar test sets are likely to detect more defects than similar 
ones \cite{Al-Hajjaji:2014:SPS:2648511.2648532}. In Fig. \ref{example1}, there are 24 legal configurations under test. This set is then narrowed down to 20 by the 4-wise algorithm.
%
By SP, the configuration with the maximum number of features is selected to be the first 
one under test where \texttt{TWL4030\_CORE, IRQ\_DOMAIN, OF\_IRQ}, and \texttt{OF\_DEVICE} are 
enabled, and \texttt{SPARC} is disabled. The next one is the configuration
that has the minimum number of similar features as the previously selected ones, where \texttt{TWL4030\_CORE}, \texttt{IRQ\_DOMAIN}, \texttt{OF\_IRQ}, and \texttt{OF\_DEVICE} are disabled, and \texttt{SPARC} is enabled. 
%For the running example, 
Although the second variant is most dissimilar compared to the first one, 
there is no bug revealed by the second. Hence, the resulted schedule is not an efficient
testing order because the run-time and compile-time bugs are not detected 
until the 4$^{th}$ and 6$^{th}$ variants are tested respectively, while the variant with both bugs would only be discovered via the 7$^{th}$ one.
%
%Another issue of SP is that the quality of the resulted order is 
%strongly depended on the selection of the first configuration.
%
Another issue of SP is that the quality of the resulted order is 
strongly depended on the first selection.
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{example_src_3.png}
\caption{A simplified buggy version of Linux kernel}
\label{example1}
\end{figure}

\noindent \textbf{Observation}. If we consider the declaration of
\texttt{of\_platform\_popu\-late} in \texttt{L} (line 5) and its use
in \texttt{Z} (line 24), the configuration which enables
\texttt{Z} and disables \texttt{L} (\texttt{CONFIG\_OF\_DEVICE=T,
  CONFIG\_SPARC=T}) should be tested earlier to detect the first
interaction bug. 
%Based on this observation, the nature of interactions
%between features should be comprehended to schedule an order of
%configurations under test to quickly discover interaction bugs.


%However, this do not mean that for a given set of 
%configurations with a certain number of bugs, the dissimilar order detect bugs faster than 
%other schedules. Especially, for the bug that is only exposed in the configuration that is much different
%from the first configuration. Indeed, for the running example, the variants that cover the second bug
%and both two bugs have low ranks, 6$^{th}$ and 7$^{th}$ respectively, while the first one is covered by the 
%4$^{th}$ variant.
%
%However, this is an inefficient 
%testing order because the run-time and compile-time errors are not observed and fixed 
%until the 4$^{th}$ and 6$^{th}$ variants is tested respectively, while the configuration 
%with both interaction bugs would only be discovered in the 7$^{th}$ variant.

%\input{kway}


==> peval.tex <==
\section{Empirical Evaluation}
We compare {\tool} against SP and random prioritization when we run them on the results of 4 advanced sampling methods \cite{Medeiros:2016:CSA:2884781.2884793}. 
We use the Variability Bugs Database~\cite{Abal:2018:VBH:3177743.3149119} with 98 real-world, verified configuration-related bugs in different versions of configurable systems. We select 46 buggy versions that have bugs not related to pointers or external data.
%
We run each sampling method on each version separately to select a subset of valid configurations, which is the input of the prioritization performed by the three methods. The output schedules of the methods are then evaluated via two metrics Average Percentage Faults Detected (APFD) \cite{962562} and average rank (AVGR). The higher APFD and the lower AVGR, the better schedule.
%

\input{comparison_apfd_src}

Table \ref{apfd_table} shows the average APFD and average rank for the three approaches. As seen, {\tool} achieves about 20\% higher APFD on average, and is able to rank the buggy configuration in a much higher rank than SP and random approaches. 

%While using VBDb, we were able to use {\tool} detect 17 interaction bugs (2 of them were reported by the developers) that were not discovered in those configurable systems and in VBDb database.

%In other words, if we add {\tool} as the prioritization technique on top of a selection algorithm, 
%we would achieve a more effective solution than adding the other approaches upon the algorithm.
%Linux, Apache HTTPD, Marlin and BusyBox.
%\input{comparison_table}


==> results1.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{copo_alltrue}
\caption{CoPo .vs \textit{All-true} approach}
\end{figure}

